Learning Generalizable Behavior via Visual Rewrite Rules

Though deep reinforcement learning agents have achieved unprecedented success in recent years, their learned policies can be brittle, failing to generalize to even slight modifications of their environments or unfamiliar situations. The black-box nature of the neural network learning dynamics makes it impossible to audit trained deep agents and recover from such failures. In this paper, we propose a novel representation and learning approach to capture environment dynamics without using neural networks. It originates from the observation that, in games designed for people, the effect of an action can often be perceived in the form of local changes in consecutive visual observations. Our algorithm is designed to extract such vision-based changes and condense them into a set of action-dependent descriptive rules, which we call ''visual rewrite rules'' (VRRs). We also present preliminary results from a VRR agent that can explore, expand its rule set, and solve a game via planning with its learned VRR world model. In several classical games, our non-deep agent demonstrates superior performance, extreme sample efficiency, and robust generalization ability compared with several mainstream deep agents.

==> figures/archived/exp_corr.tex <==
\begin{figure}[tbp]
  \centering
  \includegraphics[width=\linewidth]{figures/pdfs/expectation_correction.png}
  \caption{Learning Visual Rewrite Rules. Top figure captures a local state change ($s^t \neq s^{t+1}$). Bottom figure illustrates the absence of a state change ($s^t = s^{t+1}$).}
  \label{fig:exp_corr}
\end{figure}
